COUPA: An Industrial Recommender System for Online to Offline Service Platforms

Aiming at helping users locally discovery retail services (e.g., entertainment and dinning), Online to Offline (O2O) service platforms have become popular in recent years, which greatly challenge current recommender systems. With the real data in Alipay, a feeds-like scenario for O2O services, we find that recurrence based temporal patterns and position biases commonly exist in our scenarios, which seriously threaten the recommendation effectiveness. To this end, we propose COUPA, an industrial system targeting for characterizing user preference with following two considerations: (1) Time aware preference: we employ the continuous time aware point process equipped with an attention mechanism to fully capture temporal patterns for recommendation. (2) Position aware preference: a position selector component equipped with a position personalization module is elaborately designed to mitigate position bias in a personalized manner. Finally, we carefully implement and deploy COUPA on Alipay with a cooperation of edge, streaming and batch computing, as well as a two-stage online serving mode, to support several popular recommendation scenarios. We conduct extensive experiments to demonstrate that COUPA consistently achieves superior performance and has potential to provide intuitive evidences for recommendation

==> 9-sec-app.tex <==
\appendix
\section{Supplement}
In the appendix, we  present some details omitted in the main paper to enhance the reproducibility, including detailed descriptions about datasets, baselines and metrics. 
%Next, we show more additional data analysis results to support the motivations in our paper.


\subsection{Dataset Descriptions \label{app-data}}
For the three datasets (\ie \textbf{Food Delivery}, \textbf{Travel} and \textbf{Channel} dataset), we extract the interaction records from ``2021-01-07'' to ``2021-01-13'' for training and remain records on ``2021-01-13'' for test. Moreover, we leave out 200, 000 samples of training data as the validation set for parameter tuning. For each user in the extracted dataset, we collect his/her interaction records in the last three months to construct recent behaviors. We only preserve the users who have more than 10 behaviors and keep the ratio of positive and negative samples as 1 : 6. Also, abundant features are extract to effectively characterize users, items and associated scenarios, which have been presented in the Section 4 of the main paper.

\subsection{Baseline Descriptions \label{app-base}}
In our experiments, we compare our approach with several state-of-the-art baselines as below:

\begin{itemize}
    \item \textbf{DeepFM~\cite{guo2017deepfm}} : It is a typical feature based recommendation methods consisting of a factorization machine (FM) component and a deep neural network (DNN) component.  
    \item \textbf{GRU4Rec~\cite{hidasi2015session}} : It is a sequential recommendation method with RNN structured GRU part for user behaviors modelling.
    \item \textbf{DIN~\cite{zhou2018deep}} : It is a sequential recommendation method with attention mechanism to exploit related user behaviors. 
    \item \textbf{DIEN~\cite{zhou2019deep}} : It an improved version of DIN by considering the interest evolving process through GRU with attention update gate.
    \item \textbf{SASRec~\cite{kang2018self}} : It a representative sequential recommendation method using a left-to-right Transformer module to capture user behaviors. 
    \item \textbf{Time-LSTM~\cite{zhu2017next}} : It is a temporal recommendation method, equipping LSTM structure with time gates for time interval modelling.
    
    \item \textbf{YoutubeRank~\cite{zhao2019recommending}}: It is a industrial video ranking system for Youtube, which employs the the Multi-gate Mixture-of-Experts to optimize multiple ranking objectives and adopt a Wide\&Deep framework for mitigating the selection bias.
    
    \item \textbf{PAL~\cite{guo2019pal}}: It is a position bias aware learning framework for CTR prediction, which jointly and simultaneously optimizes the probability that a user see and click  a target item.
\end{itemize}

\subsection{Implementation Details \label{app-impl}}
We implement all methods on parameter server based distributed learning systems~\cite{zhou2017kunpeng} with Tensorflow 1.3. All parameters for baselines are optimized in the validation set as mentioned above, and we briefly present the optimal parameters in ousa experiments for reproducibility. For all methods, we perform Adam for optimization with learning rate 1e-4. We set embedding size of each feature as 8 and set the architecture of MLP as [256, 128, 64]. For sequential methods, the max length of sequence is set as 50. For SASRec, two self-attention blocks are used. We run each method ten times and average the results as the final performance

\subsection{Metrics descriptions \label{app-metrics}}
%\textbf{Offline metrics.} 
To evaluate the offline performance (\ie Section 6.3.1), we adopt the group weighted area under curve (\textbf{GAUC}), which is derived from the classical metric: area under curve (\textbf{AUC}). Formally, we can calculate the GAUC as follows:
\begin{equation}
\text{GAUC} = \frac{\sum_g{w_g \times \text{AUC}_g}}{\sum_g{w_g}}, 
\end{equation}
where $w_g$ is the weight of group $g$ (\ie the number of samples in group $g$) and AUC$_g$ is the AUC for group $g$.
Moreover, we also report the relative improvement (\textbf{RI}) \wrt GAUC of our approach over compared baselines, which is defined as:
\begin{equation}
    \text{RI} = \frac{|\text{GAUC}_{ours} - \text{GAUC}_{base}|}{\text{GAUC}_{base}} \times 100\%,
\end{equation}
where $|\cdot|$ is the absolute value, $GAUC_{ours/base}$ refers to the performance of our approach and corresponding baselines, respectively.

% \textbf{Online metrics.} To evaluate the online performance (\ie Section 6.3.2 and 6.4), we use the metrics \textbf{CTR} and \textbf{PCTR}, which are commonly adopted in various industrial online systems. 
% In particular, UCTR and PCTR can be calculated as follows:
% \begin{equation}
%     \text{UCTR} = \frac{\text{Unique\ click}}{\text{Unique\ visitor}}, \ \ \ \ \text{PCTR} = \frac{\text{Page click}}{\text{Page visitor}}.
% \end{equation}


% \begin{figure}[t]
% \centering
% \subfigure[]{
% \includegraphics[width=40mm,height=30mm]{figure/kouele_data.pdf}
% }
% %\hspace{30pt}\includegraphics[width=40mm,height=30mm]{figure/case_time.pdf}
% \subfigure[]{

% \includegraphics[width=40mm,height=30mm]{figure/column_data.pdf}
% }
% \caption{An macro analysis of the position bias on contents (\ie Koubei and Eleme) and columns. \label{fig-app-data}}
% \end{figure}

% \subsection{Additional observation for position bias \label{app-pd}}
% In the main paper, we have already analyze the users' preference towards positions in a micro view. Here, we focus on the macro view and plot the CTR distributions \wrt different positions for both columns and contents under ``Eleme'' and ``Koubei'' columns in Figure~\ref{fig-app-data} (c) and (d). Here, we calculate the positions of contents as follows,
% \begin{equation}
%     pos_{cont}=num\cdot{pos_{col}+k}
% \end{equation}
% where $pos_{col} = 0, 1, 2, ...$ denotes the displayed position of column related to the content, $num$ denotes the number of contents under corresponding column ($num=3$ for most columns) and $k = 0, 1 ,..., num)$ denotes displayed position of contents under column.
% Overall, we observe that CTR declines sharply from higher positions to lower ones, which is consistent to the findings discussed in \cite{zhu2017next, guo2019pal, richardson2007predicting}. It is worthwhile to note that the CTR for columns at the first position prominently lower than others in our scenarios, which is attributed to that a number of users enter Alipay just for payment, and thus large amounts of invalid exposures for column at the first position are caused. 

